On Small Satellites for Oceanography: A Survey

The recent explosive growth of small satellite operations driven primarily from an academic or pedagogical need, has demonstrated the viability of commercial-off-the-shelf technologies in space. They have also leveraged and shown the need for development of compatible sensors primarily aimed for Earth observation tasks including monitoring terrestrial domains, communications and engineering tests. However, one domain that these platforms have not yet made substantial inroads into, is in the ocean sciences. Remote sensing has long been within the repertoire of tools for oceanographers to study dynamic large scale physical phenomena, such as gyres and fronts, bio-geochemical process transport, primary productivity and process studies in the coastal ocean. We argue that the time has come for micro and nano satellites (with mass smaller than 100 kg and 2 to 3 year development times) designed, built, tested and flown by academic departments, for coordinated observations with robotic assets in situ. We do so primarily by surveying SmallSat missions oriented towards ocean observations in the recent past, and in doing so, we update the current knowledge about what is feasible in the rapidly evolving field of platforms and sensors for this domain. We conclude by proposing a set of candidate ocean observing missions with an emphasis on radar-based observations, with a focus on Synthetic Aperture Radar.

==> survey_OLD.tex <==
\section{Survey of SmallSats}
\label{sec:Survey}

%%\begin{itemize}
	%%\item Summary of what has been done
	%%\item Description of the small satellite systems
	%%\item Tables with relevant data
%%\end{itemize}

In this section we summarise the spacecrafts (micro or nano) that support oceanography somehow (e.g. by monitoring traffic). The ones here described were found using available online databases (the Earth Observation Portal\footnote{\url{https://directory.eoportal.org/web/eoportal/satellite-missions}}, the Union of Concerned Scientist satellite database\footnote{\url{http://www.ucsusa.org/nuclear-weapons/space-weapons/satellite-database.html}}, and the Nanosatellite Database\footnote{\url{http://www.nanosats.eu/}}), and through a search of the web. When ever possible, references of the mission (mostly papers) were used, although some information comes from the databases descriptions.

% ---------------------------------------------
% ---------------------------------------------
\subsection{Ocean Imaging}
\label{subsec:Ocean_Imaging}

Many imaging nano and micro satellites exist, and although one could argue that some of the images of the SmallSats could be use for oceanographic studies, just a few are truly focused in ocean observation. No CubeSats were found that had ocean imaging systems, as mention already in 2012 in Ref. \cite{Selva2012}, although in 2013 COPPER was close to be the first one. Of the micro satellites only two (that were already launched) were found, and one is for commercial purposes (WINISAT-1) and the other uses the data acquired for other purposes to monitor ocean health (QSat-EOS). Finally, a spacecraft that is currently being developed is discusses as it will have a dedicated ocean observation payload.

% ---------------------------------------------

\paragraph{COPPER} The Close Orbiting Propellant Plume and Elemental Recognition CubeSat was an experimental mission to study the ability of commercially available compact uncooled microbolometer arrays to take infrared Earth images (of oceans and atmosphere), besides providing a space situational awareness \cite{Massey2012}. Additionally it was intended to improve models of radiation effects on electronic devices in space. It was part of the Argus program, a proposed flight program of a few CubeSat spacecrafts spanning many years, of which COPPER was the pathfinder mission \cite{COPPER_EOPortal}. It was launched in November 2013, but communications were never established.

The spacecraft had a mass of $1.3\,\unit{Kg}$ and a $2.2\,\unit{W}$ nominal daily power. It was student built, using a 1U ($10 \times 10 \times 10\,\unit{cm}$) Skeleton CubeSat Kit (RevD), with a PIC-24 based microcontroller. For power it used, a ClydeSpace Lithium-polymer battery, and a body mounted solar cells (from SpectroLab). Attitude determination and control was performed using permanent magnets (which align the satellite with Earth's magnetic field lines) and with hyteresis rods (to dampen oscillations) \cite{Massey2012}. In terms of communications it had a UHF/VHF transceiver, using a frequency of $2.4\,\unit{GHz}$ for primary communications, and a $440\,\unit{MHz}$ beacon.

As payload the spacecraft carried the Tau LWIR (Long Wave Infrared) camera, which was a microbolometer array, and the Commodore experiment, a small printed circuit board to monitor event (radiation particle collision) data.

% ---------------------------------------------

\paragraph{WNISAT-1} One of the largest weather companies, Weathernews Inc. of Tokyo, funded the sea monitoring mission WNISAT-1 (Weathernews Inc. Satellite-1), which was launched in 2013 \cite{AXELSPACECooperation2013}. The objective was to provide data on the Arctic Sea state to shipping customers operating on that area \cite{Kim2010}. The nano satellite was designed by a university venture company, AXELSPACE. The intention was to use a simple architecture, and where possible with commercial off the shelf (COTS) devices with a compact design simple operational support, and minimum redundancies. 

The adopted model was a cubic shape of $27\,\unit{cm}$ of side, with a launch mass of $10\,\unit{kg}$, and a design life of two years. The bus panels are of aluminium, and a passive thermal control is employed. For this mission the attitude pointing is not very stringent (as the pixel size of the camera is large, $500\,\unit{m}$), and the resources are limited. As such, the three axis stabilization is performed through a magnetic torque rod, and four reaction wheels. The attitude determination is provided by a magnetometer, three gyroscope, four sun sensors, and two star trackers. To determine its orbit the satellite uses a GPS receiver. In terms of power the spacecraft generates in average $12.6\,\unit{W}$, through solar cells mounted on the surface (in five sides of the cube). A Li-ion battery with a capacity of $7700\,\unit{mAh}$ provides power during eclipses. To communicate with Earth a UHF band was selected, and five antennas were installed (one to receive, and remaining to transmit). This arrangement provides stable communications while minimising shadow effects.

The payload of the WNISAT-1 are two cameras, one for the visible radiation spectrum (VIS) and one for the near infrared (NIR). Both cameras use the same optical system and CMOS detector type, and
monitor ice state. The ground sample distance is $500\,\unit{m}$, with a snapshot size of $500\,\unit{km}$, and ten scenes per day taken \cite{Kim2010}.

There is also a laser installed to measure CO$_2$ density in the atmosphere. This works by emitting two laser beams (with $1570\,\unit{nm}$ and $1556\,\unit{nm}$) which are then measured by a ground station (and from the strength of the signal a CO$_2$ concentration is derived). An important aspect is that the laser pulse peak power requirement is much higher than the capacity of the satellite (output power between $500$ and $5\,\unit{kW}$ with a frequency between $500\,\unit{Hz}$ and $10\,\unit{kHz}$) \cite{Kim2010}. To overcome this situation the measurement period is very short and the unit is equipped with a separate battery package.

% ---------------------------------------------

\paragraph{QSat-EOS}: Graduate students of Kyushu University, in Japan, started developing a spacecraft for space science. However, due to funding requirements the main objective of the mission was shifted to Earth Observation, in particular disaster monitoring, monitoring of Earth's magnetic field, detection of micro debris, and observation of water vapour in the upper atmosphere \cite{QSatEOS_EOPortal,Aso2011}. The data acquired is also expected to support other studies, namely agricultural pest, red tide, and ocean eutrophication (i.e. a type of pollution due to excess of nutrients \cite{Wallace2014}). 

Launched in 2014, the spacecraft, made of an aluminium alloy, has a mass of about $50\,\unit{kg}$, with dimensions around 50 cm in each side of the cube (although it has a de-orbit sail mechanism which when deployed measures 3 x 0.4 m). Power generation is of the order of $70\,\unit{W}$, using 200 body-mounted solar cells. The rest of the electric power subsystem consist in a power unit and $10.5\,\unit{Ah}$ NiMH (Nickel Metal Hydride) battery unit (which basically is 18 AA batteries), and supplies a bus voltage of $7.2\,\unit{V}$. The satellite's attitude is determined with six sun sensors, a three axis magnetometer, two star trackers, and a fibre optic gyroscope, while a GPS gives orbital position. Three axis attitude control is achieved using magnetic torquers and reaction wheels. Telemetry and command communications (up and downlink) is performed through S-band (two antennas). The payload data is downlinked by a Ku-band antenna (and an experimental uplink also uses this antenna).

For the secondary objectives (debris detection and magnetic field monitoring), the satellite has a debris sensor and uses the magnetometer. Conversely, a two band visible and near infra red camera is installed to accomplish the mission's primary objective (and which will also be used for investigating ocean eutrophication). This is an optics with a aperture diameter of $100\,\unit{mm}$ (and focal length of $400\,\unit{mm}$), linked to a CMOS detector (resolution of about $5\,\unit{m}$ and 2000 x 2000 pixels) that will read two spectral bands (525 to 605 nm and 774 to 900 nm). The field of view for a reference altitude of $700\,\unit{km}$ is a square of $10\,\unit{km}$ side.

% ---------------------------------------------

\paragraph{RISESat} The Rapid International Scientific Experiment Satellite (RISESat) is being developed under an international cooperation lead by Tohoku University, within the Japanese FIRST (Funding Program for World-Leading Innovative R\&D on Science and Technology) program \cite{Kuwahara2012}. With a launch planned for 2016, the objectives are two fold, technological --  to demonstrate the platform performance, as it is planned to be a common bus for future missions -- and scientific -- integrating scientific payloads from different countries, mainly focused on Earth and its environments (to a total of about $10\,\unit{kg}$) \cite{RISESat_EOPortal}. The payloads include a High Precision Telescope (HPT), a Dual-band Optical Transient Camera (DOTCam), a Ocean Observation Camera (OOC), a Three-dimensional Telescope (TriTel), a Space Radiation micro-Tracker (Timepix), a micro-Magnetometer ($\mu$MAG), a Very Small Optical TrAnsponder (VSOTA), and a Data Packet Decoder (DPD).

The spacecraft bus was named Advanced Orbital Bus Architecture (AOBA), as it is intended to be versatile, cost effective, and with a short development schedule, to be compatible (and competitive) for future scientific missions. Therefore, the size of the bus has to be smaller than 50 x 50 x 50 cm, with a maximum mass equal to $60\,\unit{kg}$ (but typical less than $55\,\unit{kg}$). The main structure has a central squared pillar, with one side extended to connect to the outer panels (increasing the mounting surface, and resulting in a more stable satellite). The outer panels are made of an aluminium isogrid. 

Attitude determination is performed through the use of two star sensors, a three axis fibre optic gyroscope, a magnetometer also of three axis, a GPS receiver, and coarse and accurate sun sensors (covering 4$\pi$). Whereas control is achieved with four reaction wheels and three axis magnetic torquers. To have a high reliability, some sensors and actuators are designed in a redundant form.

Power is supplied by GaAs multijunction cells, mounted in two deployable panels and one body mounted, generating more than $100\,\unit{W}$. The enhanced amount of electric power, around double the power consumption (as the expected one is more than $50\,\unit{W}$), allows for long period and multi instruments observations. A power control unit provides each subsystem supply lines, although some more demanding components (in terms of power) are also directly connected to the PCU. Also part of the electric subsystem are the batteries, which are NiMH type batteries ($3.7\,\unit{Ah}$ and $18\,\unit{V}$).

Three different bands are used for communications. The UHF is used for command uplinks, at a maximum rate of $1.2\,\unit{kbps}$, and a S-band for housekeeping downlink (with a maximum rate of $38.4\,\unit{kbps}$). As large amounts of scientific data are expected to be generated, another downlink system was added with a maximum rate of $2.45\,\unit{Mbps}$ (using a X-band system) \cite{RISESat_EOPortal}.

Furthermore, a de-orbit mechanism (DOM) will be installed, to make the spacecraft re-enter Earth in about 25 years, following the United Nations suggestions. Six micro cameras will also be installed to monitor the satellite's structure and deployment, and to view the Earth and where the instruments are pointing to. All payloads have a remote terminal unit to interface with the spacecraft bus system.

As this paper is focused on oceanography we describe here in more depth just the Ocean Observation Camera, and just give a brief description of the other payloads. The OOC is a multi-band camera (about $100\,\unit{m}$ pixel resolution) with a wide field of view (swathe width of approximately $65\,\unit{km}$) \cite{Kuwahara2012}. Although the system will work in a continuous acquisition mode, the interest target area is the regions around Japan and Taiwan. The resulting data will be mainly used for the fish industry and environment studies. It is compatible to the Space Plug \& Play (SPA) technology, and has a mass of about $1\,\unit{kg}$ \cite{RISESat_EOPortal}. Furthermore, it has a power consumption of less than $3\,\unit{W}$, and uses a Watec T065 CCD (charge-coupled device) with 659 x 494 pixels (square pitch size of $7.4\,\unit{µm}$), for each F/1.4 lens.

The HPT will be used to take multi-spectral images of both Earth and for astronomical observations. The DOTCam is in turn focused on observation of TLEs (Transient Luminous Events) in Earth's upper atmosphere. Aiming at identifying the LET (Linear Energy Transfer) spectrum and the quality factor of cosmic radiation, the TriTel measures energy deposits of charged particles. Also directed to radiation studies, the Timepix instrument intends to characterise the mixed radiation field of a Low Earth Orbit (i.e. the entire charged particle spectrum, including energetic electrons, protons, and relativistic cosmic-ray ions). The $\mu$MAG, as the name suggests, is a magnetometer using MEMS technology. To test one-way optical communication between the spacecraft and a ground station, that pretends to achieve at least $100\,\unit{kbps}$ when transmitting to a $1.5\,\unit{m}$ diameter telescope, RISESat uses the VSOTA instrument -- which will downlink payload data. Finally, the DPD is a simple store-and-forward device to collect data from in-situ measurement instruments and transmit it to ground stations (a technology inherit from the WEOS micro satellite).

% ---------------------------------------------

%%\paragraph{CanX-1}\footnote{\url{https://en.wikipedia.org/wiki/Canadian_Advanced_Nanospace_eXperiment_Program}}
%%The Canadian Advanced Nanospace eXperiment (CanX) was a pico-satellite
%%(10X10X10cm) and 1 kg mass student demonstrator, used primarily to
%%test concepts and technologies for future flight \cite{canx}. With a
%%low powered onboard computer with a CMOS imager, GPS receiver and COTS
%%magnetometers for attitude control as the primary payload, it was
%%launched June 2003 but promptly lost contact. An early experiment, it
%%was followed by other pico-satellites in the series (CanX 2 thru 5)
%%with active propulsion and used to demonstrate formation flying.
%%
%%
%%\paragraph{CP1}\footnote{\url{http://polysat.calpoly.edu/launched-missions/cp1/}}
%%California Polytechnic Institute (CalPoly) students built their first
%%satellite as a demonstrator with the primary payload being a small
%%commercial sun-sensor and a magnetic torquers for attitude control
%%\cite{cp1}. The 2006 launch of the satellite failed, as did a
%%succession of other cubesats from this group, till CP-5 and beyond
%%were launched and operated nominally. Current versions of their
%%SmallSats carry payloads for weather observation and image processing.
%%CalPoly is considered to be the early innovator in SmallSats.


% ---------------------------------------------
% ---------------------------------------------
\subsection{Constellations}
\label{subsec:Constellations}

Constellations can be considered a category on their own. The idea behind it is by combining several observations of the same observable, perform from different platforms (each one considered a SmallSat), we can have scientific data that could not be acquired using a single spacecraft (or at least with better quality).

An example of this is the CYGNSS (Cyclone Global Navigation Satellite System) constellation. Each satellite has a mass of $25\,\unit{kg}$ (i.e. it is a micro satellite), but the constellation has eight identical satellites weighting in total $200\,\unit{kg}$ \cite{CYGNSS_EOPortal}. This constellation, expected to be launched in 2016 in a single rocket, will serve to relate ocean surface properties (retrieved from reflected GPS signals), atmospheric conditions, radiation and convective dynamics, to tropical cyclone formation. 

Another example is the SOCON (Sustained Ocean Observation from Nanosatellites) project, which intends to develop the SeaHawk spacecrafts (3U CubeSats) \cite{SeaHawk_GunterSpace}. Two prototypes are expected to be launch in 2017, and will act as forerunners for the constellation of ten SmallSats, that has the objective of measuring ocean colour (using HawkEye Ocean Colour Sensors). The associated cost is expected to be about eight times less (with a resolution seven to 15 times better) than its predecessor, the single mini satellite OrbView-2 (SeaStar).


% ---------------------------------------------
% ---------------------------------------------
\subsection{Data Relay Satellites}
\label{subsec:Data_Relay}

There are missions that do not have payloads design specifically for oceanographic studies, but even so perform/support oceanography studies, as is the case of data relay spacecrafts. In other others, these spacecrafts receive data from in-situ experiments (for instance buoys) and transmit the data received when in view of a ground station. This way a human operator does not have to be close by the experiment, or constantly visit it, to get the acquired data. An example case were this capability is important is the Whale Ecology Observation Satellite (WEOS) of the Chiba Institute of Technology in Japan.

Other satellites examples within data relay satellites are the ParkinsonSat \cite{ParkinsonSat_EOPortal}, the TUBSAT-N and N1 (Technical University of Berlin Satellite-Nano) nano spacecrafts (which were launched from a submarine) \cite{TUBSAT_EOPortal}, the twin CONASAT $8.2\,\unit{kg}$ spacecrafts \cite{Carrara2014}, and the FedSat (Federation Satellite) \cite{Fedsat_EOPortal}.

% ---------------------------------------------

\paragraph{WEOS} Launched in 2002, to a sun-synchronous orbit of about $800\,\unit{km}$, the WEOS spacecraft was designed, built and operated by students, with the goal of tracking the signals emitted by probes attached to whales. This would allow to study the migration routes of whales. The probe transmitted several informations (including GPS position, diving depth, and sea temperature) using the UHF band \cite{Hayashi2004}.

The spacecraft weights about $50\,\unit{kg}$, and measures 52 x 52 x 50 cm. It has a deployable gravity-gradient boom, to stabilised the satellite and keep the antenna facing the Earth, with a length of $3\,\unit{m}$ and a $3\,\unit{kg}$ tip mass. Attitude is controlled also using a three axis magnetic torquer, and determined by a also three axis flux gate magnetometer and a GPS receiver. A S-band transmitter ($1.2\,\unit{kbps}$) and a UHF receiver (data rate $300\,\unit{bps}$) are used for communications and gathering of data from the whales probes. The power subsystem consists of body mounted Si crystal solar cells (generating on average $14.5\,\unit{W}$), NiCd batteries (with a capacity of $4\,\unit{Ah}$), and a power control unit. A central computer controls all the spacecraft operations \cite{Hayashi2003}.


% ---------------------------------------------
% ---------------------------------------------
\subsection{Tracking and the Automatic Identification System}
\label{subsec:AIS}

\rever{Description of AIS system -- Does it need to be expanded?}

Maritime domain awareness is a key need for governments and policy makers worldwide. Within Canada's extended continental shelf approximately 1600 ships transect per day \cite{Bedard2007}. Japan and Norway are other two examples of countries which took careful attention to maritime traffic, as their exclusive economic zones are vast \cite{Eriksen2010a,Nakamura2013}.

Most ship monitoring is currently performed using maritime radars and by ground based Automatic Identification System (AIS) \cite{Orr2013}. The AIS system is mandatory for all ships with more than $300\,\unit{tonnes}$, and all passenger ships, and it is essentially a VHF signal consisting primarily of, the Maritime Mobile Service Identity, the position, heading, time, rate of turn, and cargo \cite{Bedard2007}. AIS is primarily to avoid collisions and provide maritime domain awareness and traffic control, with transmission from ship to ship or ship to shore \cite{Orr2013}. The monitoring done on shore, limits the detection range to about $37-74\,\unit{km}$, making it only practical for ports and in maritime choke points.

Some problems exist when putting a AIS receptor in space. The AIS system is self organized and usually within $100\,\unit{km}$ (typical range of the signal) the system organises the ships so not to have overlaps. However, due to the wider field of view of a space-based platform, there are problems of collision of signals from ships, especially in high traffic areas \rever{citation}. Another problem is the high relative velocity of the spacecraft, which induces Doppler shifts \cite{Nakamura2013}. Furthermore, the ionosphere induces a Faraday rotation of the polarization plane of the signals.

A significant part of the time is spent in identifying if unknown targets, collected from a variety of Intelligence, Surveillance, and Reconnaissance (ISR) sensors, are friendly or are of interest. An efficient process to perform this sorting, and to correlate information with other ISR data, is critical. A possibility, suggested by many authors is the combination of the AIS with SAR.

Next we describe some of the spacecrafts to which there is plenty of information on the databases used.

% ---------------------------------------------

\paragraph{AAUSat}: The Department of Electronic Systems of Aalborg University (AAU) created a educational program were students could have access to many aspects of satellite design and development. From this program three satellites were designed for tracking vessels with AIS systems, the AAUSAT3, AAUSAT4 and AAUSAT5 \cite{AAUSAT_Page}. OF these, the AAUSAT3 has finished its mission, the AAUSAT5 is soon to be launched from the ISS (International Space Station), whereas AAUSAT4 is still in a test phase. With each spacecraft a new version of the AIS system is flown. The AAUSAT3 takes two types of AIS systems, a conventional hardware receiver, and a software defined radio (SDR) based receiver. The latter one allows to update the algorithms used in the system.

AAUSat3 is a standard 1U CubeSat, with a mass of just $0.8\,\unit{kg}$, while AAUSAT5 is slightly heavier ($0.875\,\unit{kg}$) \cite{AAUSAT_Page,AAUSat3_EOPortal}. The electronic power supply (EPS) subsystem is composed of a power conversion unit (PCU), which has a student designed maximum power point tracking (MPPT) algorithm, a power regulation unit (PRU), and a power distribution unit (PDU). These three units are linked to the photo-voltaic cells, batteries, and the spacecraft bus. The AAUSat3 has five triple junction solar cells, each can provide $1.15\,\unit{W}$, and a pack of two Li-Ion batteries, which together supply $8.2\,\unit{V}$ and $2,2\,\unit{Ah}$. Conversely, AAUSat5 has twelve solar cells, and the batteries have each $3.7\,\unit{V}$ $2.6\,\unit{Ah}$. Both spacecrafts use UHF for uplink and downlink communications. The attitude determination and control subsystem is divided in two parts in the AAUSat3. One part exploits the magnetic field for main detumbling (i.e. to stabilise the angular rate of the satellite after orbital insertion), using a compass (to measure the magnetic field) and six coils to actuate. The other part is a more conventional attitude determination, utilising six sun sensors, a three axes gyroscope, and a three axis magnetometer. Most subsystems are controlled through a Atmel microcontroller, while the strictly sensing part of the attitude determination has a ARM7 microcontroller.

% ---------------------------------------------

\paragraph{LambdaSat}: A group of international students in Silicon Valley in the USA, have developed a spacecraft with three main objectives: space qualification of graphene when direct exposed to solar radiation and space; demonstration of an AIS system; space qualification of three-fault tolerant spacecraft; and finally address educational objectives \cite{Mantzouris}. The spacecraft was named Lambdasat ($\Lambda$-sat), in honour of the Greek professor which proposed the mission, and was deployed in 2015 from the International Space Station \cite{LambdaSat_EOPortal}.

The spacecraft was designed respecting 1U CubeSat dimensions, using a structure of Pumpkin, Inc. of San Francisco, but when deployed unfolds body mounted solar arrays, passing to a 3U envelope. The power system and the main computer were designed and built for this spacecraft in particular (to fulfil the third objective). Communications are performed over UHF and using the Iridium satellite constellation.

Payloads include the AIS receiver and equipment to measure radiation effects on the graphene material.

% ---------------------------------------------

\paragraph{ZACube-2}: The Cape Peninsula University of Technology (CPUT) created a program to develop nano satellites in South Africa, of which the ZACube-2 will be the second spacecraft \cite{Villiers2015}. This spacecraft will serve as a technology demonstrator including a software defined Radio (SDR), which will be used for tracking AIS signals, and a medium resolution imager (as a secondary payload), to perform ocean colour and large fires monitoring.

A 3U CubeSat platform, based on the Clyde Space design, is deemed as the most appropriate to accommodate all the subsystems, and at the same time provide enough surface area for the body mounted solar panels. For command and data handling several processors will be present, while for communications a UHF transceiver developed in-house will be used. A S-band transmitter will be necessary for downlink of the image collected and AIS signals.

As mentioned before the end of life of spacecrafts must be addressed when designing one, to comply with United Nations (UN) policies (which state that a satellite must re-enter the atmosphere within 25 years after the end of the mission). In this satellite in particular, its deorbiting device is a Terminator Tape (developed by Tethers Unlimited). It has a mass of just $0.083\,\unit{kg}$ and deploys when the mission is complete, becoming a 10 x 8.3 x 0.65 cm conducting tape (generating neutral particle and passive electrodynamic drags).

% ---------------------------------------------

\paragraph{NTS/CanX-6}: In 2007/2008 a cooperation between the University of Toronto, Institute for Aerospace Studies/Space Flight Laboratory (UTIAS/SFL) and COM DEV Ltd, designed, produced and launched a nano satellite to perform experiments in the reception of AIS signals in space, in less than seven months, the Nanosatellite Tracking Ships (NTS) \cite{Pranajaya2010a}. While the platform is based on SFL CanX-2 nano satellite and the Generic Nanosatellite Bus (GNB), the AIS payload was developed by COM DEV Ltd. A top-down approach was performed, based on the mission requirements (lifetime, data throughput, attitude, schedule, and resources), balanced with a bottom-up analysis, which accounted for hardware limitations (on-board memory, downlink rate, power, volume, and others), maturity and readiness.

The spacecraft is an aluminium cube of $20\,\unit{cm}$ (80 x 45 x 37 cm considering the antennas \cite{Pranajaya2010}), with a mass of about $6.5\,\unit{kg}$. Six body-mounted solar panels (with triple junction solar cells) produce up to $5.6\,\unit{W}$ \cite{NTS_EOPortal}, supported by a $3.6\,\unit{Ah}$ battery. It has a housekeeping computer, with $2\,\unit{MB}$ of protected RAM and $16\,\unit{MB}$ of flash RAM, and runs the CANOE (Canadian Advanced Nanospace Operating Environment) software. Passive surface coatings are the main thermal control. A passive attitude control is also employed, with a single permanent magnet and six hysteresis rods. Six coarse sun sensors gives the satellite's attitude. Four UHF antennas are present for command and software uplink at a rate of $4\,\unit{kbps}$, whereas two S-band patch antennas downlink telemetry and data with a nominal $32\,\unit{kbps}$.

The AIS system is the single payload of the mission, and included a $46\,\unit{cm}$ antenna. With this antenna the spacecraft becomes $80\,\unit{cm}$ long, which has to be accommodated in the launch vehicle. This is solved using the XPOD GNB separation system.

% ---------------------------------------------

\paragraph{AISSat-1}: Launched in 2010 (to a $630\,\unit{km}$ altitude Sun synchronous polar orbit), the AISSat-1 is the first dedicated satellite build for space-based monitoring of AIS signals, by Norway in partnership with the University of Toronto, Institute for Aerospace Studies/Space Flight Laboratory (UTIAS/SFL) \cite{Eriksen2010a, Narheim2008}. The objective is to enhance maritime domain awareness in the Norwegian waters, which amount to more than 2 million square kilometres, and are already under surveillance using ships, coastal radars, SAR (the Canadian RADARSAT-1), and 40 AIS ground stations.

The platform has a cube shape ($20\,\unit{cm}$ side) and was developed by UTIAS/SFL, based on the modular GNB (Generic Nanosatellite Bus). With an aluminium alloy (Al 6061-T6) structure, with two internal trays that contain all the needed components for any mission \cite{AISSat1&2_EOPortal}, it has a mass of about $6.5\,\unit{kg}$, and generates up to $0.967\,\unit{W}$ with 36 body-mounted solar cells. A $5.3\,\unit{Ah}$ lithium-ion battery is used during eclipses. For communications it contains a UHF receiver ($4\,\unit{kbps}$) and a S-band transmitter (up to $256\,\unit{kbps}$).

The main payload, the AIS sensor, is a simple dual channel VHF receiver, tune to the AIS frequencies of KSX (Kongsberg Seatex AS), linked to a FPGA (field-programmable gate array). The FPGA makes it possible to process the signal on-board to fine tune the sensor, and reprogram it when future improvements appear. A GPS receiver is mostly needed to have an accurate clock for the AIS receiver.

Due to the success of the AISSat-1 mission, two more spacecrafts (almost copies of the first), the AISSat-2 and 3, where launched.

% ---------------------------------------------

\paragraph{AISat}: The Automatic Identification System Satellite (AISat) was designed by the German Aerospace Center (DLR), and launched in 2014, to monitor AIS signals. In particular, the Institute of Space Systems is responsible for adapting the Clavis bus to this mission, while the Institute of Composite Structures and Adaptive Systems developed the helical antenna for the AIS payload \cite{Block2013}. Two companies (The Sch\"{u}tze Company and Joachims) and the Bremen University of Applied Sciences were also partners in the project. The difference between this mission and others here described is the use of an helical antenna.

As stated above the AISat is an adaptation of the Clavis bus, which itself is four PC/104 CubeSat boards in a stack configuration interfaced by a back plane board (that also provides data and electrical interface) \cite{Nohka2012}. Five body-mounted solar panels, with 12 GaAs cells, that generate up to $15\,\unit{W}$, together with a $40\,\unit{Wh}$ battery, and a Power Conditioning and Distribution Unit (PCDU) make up the power system. A switching board is added to protect the bus of power failures and to switch between 3.3, 5 and $12\,\unit{V}$ \cite{AISat_EOPortal}. The solar cells are used also as sun sensors, for the attitude determination, for which a magnetometer and a gyroscope is also employed. Whereas control is achieved with magnetorquer, and the help of the fully deployed helical antenna. A omnidirectional coverage UHF system is used for downlink and uplink. The satellite has a total weight of $14\,\unit{kg}$.

The AIS payload, with its $4\,\unit{m}$ long helical antenna, is believed to precisely locate individual ships from an altitude of about $600\,\unit{km}$, even in areas with large concentration of ships (which is difficult for other space AIS systems) \cite{Block2013}. Furthermore, it is able to receive Search And Rescue signals. Since the length of the antenna is very large, compared to the spacecraft, the fact is helical is also a benefit as it needs to be compressible and stowable.

% ---------------------------------------------

\paragraph{VesselSat}: LuxSpace Sarl owns and operates two micro satellites, the VesselSat 1 (launched in 2011) and 2 (in 2012), to monitor maritime traffic with a space based AIS system \cite{VesselSat_EOPortal}. These two built upon the experience gained on the Rubin 7, 8 and 9 non-separable payloads flown before.

These are $29\,\unit{kg}$ and $30\,\unit{cm}$ cube spacecrafts. Internally it consists of three vertical plates and one honeycomb core sandwich base plate. Outer plates just cover the inside of the spacecraft and support the solar panels (five on the side and top faces). All the electronics are suspended between the plates on rails. Adding to the solar panels, a Power Control Unit (PCU) is used, and two strings of batteries. Attitude control is limited with a magnetorquer, but sensing is achieved with two sun sensors, one magnetometer, and two gyroscopes. Two tele-command, with GPS, and four UHF antennas are part of the omnidirectional communications subsystem.

The payload is a double fully independent AIS (VHF) receivers. Furthermore, in case of failure of the UHF antennas it can also be used for receiving commands.

% ---------------------------------------------

\paragraph{SDS-4}: JAXA (Japan Aerospace Exploration Agency) created the Small Demonstration Satellite program in 2006, to test next generation space technologies and, at the same time, create a standard $50\,\unit{kg}$ bus for future missions (together with other partners) \cite{Nakamura2013}. Within this program the Small Demonstration Satellite 4 (SDS-4) is the second satellite and one of its objectives, apart from demonstrate high performance and small size bus technology, is to validate a space-based AIS system \cite{Takai2013}.

The SDS-4 platform structure is made of aluminium honeycomb, its dimensions are 140 x 50 x 45 cm after deployment (when, for instance, the solar panels were extended), and has a mass of about $50\,\unit{kg}$ \cite{Takai2013}. The power load is approximately $60\,\unit{W}$. The attitude determination subsystem has five sun sensors, a magnetic sensor (which together calculate the inertial-to-body quaternion using a quaternion estimator algorithm, QUEST), a star tracker, and a MEMS gyroscope, using then an extended Kalman-filter (EKF) \cite{Nakamura2013}. The control is achieved using three reaction wheels and magnetorquers, and a zero-momentum control technique. Communications are all over the S-band and range from just $4\,\unit{kbps}$ (uplink) to $1\,\unit{Mbps}$ (for downlink of mission data). Power generation comes from GaAs solar array cells, mounted in the body of the spacecraft and two solar panels, and is stored in two Ni-MH (Nickel metal hydride) batteries (that work in parallel, having $3.7\,\unit{Ah}$) \cite{Ohtani2011}.

The objective of the AIS system on the SDS-4 is to try to solve the problems of an AIS space-based system (the collision of signals, the Doppler shift and the Faraday rotation) \cite{Nakamura2013}. The remaining payloads are: a Flat-plate Heat Pipe (FHP) On-orbit Experiment (FOX) -- to test the dissipation of heat on the spacecraft using the FHP; a Quartz Crystal Microbalance (QCM) -- for monitoring the environmental contamination of the spacecraft during its entire life cycle; and the In-flight experiment of Space materials using THERME (IST) -- an experiment with CNES (Centre national d'\'{e}tudes spatiales) to measure solar absorptance and degradation characteristics of the new thermal control materials.

% ---------------------------------------------

\paragraph{LAPAN-A2}: The Indonesian space agency (LAPAN) propelled by the training of its own engineers in the Technical University of Berlin (during the design and building of LAPAN-TUBSAT or A1), developed the LAPAN-A2 spacecraft for Earth observation, disaster mitigation, and implementation of an AIS system \cite{Hardhienata2011}.

The spacecraft is a box of 47 x 36 x 50 cm, and a mass of $68\,\unit{kg}$. A maximum power of $32\,\unit{W}$ is provided by 30 body-mounted triple junction GaAs solar cells (grouped into four panels). The Li-ion batteries, three in parallel with four cells each (in series), provide $15\,\unit{V}$ and a capacity of $17\,\unit{Ah}$ \cite{Triharjanto2012}. An enhanced attitude determination and control subsystem is employed, using three reaction wheels and magnetic torquers, laser gyroscopes, six sun sensors (coarse), redundant star trackers, and a three axis magnetometer. Orbit position is acquired with a GPS. For telemetry tracking and command uplink and downlink the spacecraft has a UHF antenna, whereas the video payload downlink is perform through S-band \cite{LAPANA2_EOPortal}.

LAPAN-A2 payloads consist of a video camera assembly (for Earth observation), an automatic packet reporting system (radio text and voice repeater to support ground communications in time of natural disasters), and a AIS system. The AIS instrument is similar to the own of AISSAT-1 \cite{Hardhienata2011}.

% ---------------------------------------------

\paragraph{M3MSat} The Canadian Department of National Defence (DND) wanted to expand the range of AIS farther than the maritime inner zone (about $90\,\unit{km}$), and integrate AIS and ISR data to produce an improved Recognized Maritime Picture (RMP) \cite{Bedard2007}. An efficient solution is a space platform. Building upon the experience of a previous mission a new satellite is
scheduled to launch in mid 2015, the M3MSat (Maritime Monitoring and Messaging Microsatellite). The main mission objectives are: to monitor ship AIS signals (utilized by the Canadian government and Exactearth a commercial venture for tracking AIS data); serve as a platform demonstrator; and establish a flight heritage \cite{Bedard2007}.

The bus is based on the Advanced Integrated Microsatellite (AIM) of COM DEV International Ltd. It has dimensions of $0.6 \times 0.6 \times 0.8 \,\unit{m}$ and mass of about $85 \,\unit{kg}$ \cite{Orr2013}. The structure is a combination of a set of panels, to which various subsystems are attached. The panels are bolted together to make the primary structure. The bus is fully redundant to single failure scenarios. The Electrical Power Subsystem (EPS) uses solar panels (triple junction GaInP/GaAs/Ge cells) mounted on the satellite's body to generate power. The panels are connected to battery charge regulators (BCRs), that track peak power and regulate battery charging. An average of $80$ to $120\,\unit{W}$ is generated by six panels. A Li-Ion battery, with 24 cells, provides power during eclipses (with a nominal voltage of $29.6\,\unit{V}$ and a capacity of $480\,\unit{Wh}$). The power distribution is performed by a pair of power distribution modules (PDMs) \cite{Orr2013}. To communicate the satellite uses four S-band receivers and transmitters (two plus two), arrange on opposite corners of the spacecraft, giving a 4$\pi$ coverage. Attitude determination is performed by two 3-axis magnetometers, two MEMS rate sensors (also three axis), and six dual axis sun sensors. To control the attitude a set of reaction wheels and magnetic torque rods (i.e. a set of electromagnetic coils produce a magnetic field that produces a torque interacting with Earth's magnetic field) are employed. The torque rods are used for the initial detumbling (i.e. stabilised the angular rate after orbital insertion), and desaturation of the reaction wheels. It also has four GPS patch antennas, to determine its position in space.

The AIS-PEM (Automatic Identification System - Payload Electronics Module) receives AIS signals transmitted by ships, and after some processing sends the signal to ground. It consist of a VHF antenna ($30\time30\,\unit{cm}$), developed by the University of Waterloo and COM DEV Ltd., several electronics, and a dedicated $20\,\unit{Mb/s}$ C-band transmitter.

The secondary payload, the LDRS-PEM (Low Data Rate System - Payload Electronics Module), is to perform two-way communications at a low data rate system to support sensor data collection, machine-to-machine communications, and other packet based messaging services. A UHF antenna collects data from small ground terminals and downlinks it using a C-band link. To demonstrate its function data from buoys placed directly in the ice equipped with an AIS receiver/transmitter will be processed.

% ---------------------------------------------

\paragraph{exactView}: The exactView spacecrafts/payloads are part of the exactEarth company constellation of currently seven AIS spacecrafts \cite{ExactEarth2015}. With this constellation exactEarth expects to have a global revisit time (gap between subsequent detection of individual ships) of around 90 minutes, giving their customers a view of traffic in an area of interest.

The first satellite was the experimental NTS (EV0), discussed above, which is considered by exactEarth to be nowdays retired of active duty. Afterwards, in 2011, came the EV2, aboard ResourceSat 2 satellite, and EV6 and 5R (which were named AprizeSat-6 and 7), produced by SpaceQuest and transfered to exactEarth. The fifth satellite, launched in 2012, is exactView1 (EV1). The AprizeSat 8 was commissioned and became EV12 in 2013. More recently, in 2014, EV11 and 13 (AprizeSat 9 and 10) started operations. Three more satellites are expected to be added to the constellation, the EV9 (to be launched in 20 of September 2015), the EV8 (which is actually a payload of the Spanish mission Paz), and the M3MSat discussed above (considered by exactEarth to be EV7) \cite{exactEarth_constellation}.

The AprizeSat constellation goes beyond the 6 to 10 that passed to exactEarth. About 64 satellites are planned, so to build a global system of data communication, assets tracking and monitoring, and in some cases AIS payloads \cite{AprizeSat_GunterSpace}. We have more data on the AprizeSat 3 and 4, although they are all very similar spacecrafts \cite{UCSDatabase2015}. Weighting around $12\,\unit{kg}$, they are a $25\,\unit{cm}$ cube of stacked aluminium trays closed by sheet metal side panels \cite{AprizeSat_EOPortal}. Power is generated by six body-mounted panels, four of which are Ultra Triple Junction GaAs, generating each $15,\unit{W}$, and two $7.7\,\unit{W}$ single string panels. Power regulation is performed by a peak-power-tracking battery charge regulator (BCR), providing 3.3, 5, and $12\,\unit{V}$ (and an unregulated $8\,\unit{V}$), and is attached to $4\,\unit{Ah}$ six NiCd cell battery.

The EV1 spacecraft has a size of 63 x 63 x 60 cm and a mass of $98\,\unit{kg}$ \cite{exactView_exactEarth}. It employs a S-band and C-band communications system, to downlink the data acquired. For power it has a deployable solar array, body-mounted solar cells, and batteries \cite{exactView1_GunterSpace}. The orbit is Sun-synchronous with a periapsis of $806\,\unit{km}$ \cite{UCSDatabase2015}.

% ---------------------------------------------

%%\paragraph{Flying Laptop}: The Institute of Space Systems of the University of Stuttgart is developing a technology demonstration mission, the Flying Laptop \cite{Lengowski2015}. Besides serving as a technology platform, it will be used for multi-spectral Earth observation (using a multi-spectral imaging camera, and a thermal infrared camera system), and carry a AIS receiver payload. It is schedule to launch around 2016, to a targeted sun synchronous $650\,\unit{km}$ altitude orbit.
%%
%%Although it had many configurations, this is a mini satellite with $120\,\unit{kg}$ and a size of about 60 x 70 x 87 cm, designed and built primarily by students. The power available will be of the order of $270\,\unit{W}$, generated by GaAs solar panels \cite{FlyingLaptop_EOPortal}. Of the demonstration technologies is a laser link terminal for data downlink, and a LEON3FT based on-board computer.

% ---------------------------------------------

There are a few spacecrafts were not much information was found besides some general data and the launch date. For instance, Triton 1 and 2 are two examples of nano satellites (3U CubeSat standard), from the UK, that have the objective of experiment advanced AIS receivers \cite{Triton_GunterSpace}. TianTuo 1 is a Chinese nano satellite ($9.3\,\unit{kg}$) from the National University of Defense Technology (NUDT) that also performs tracking of AIS signals, besides other experiments \cite{TT1_GunterSpace}. Another two that there is not much information available are Perseus-M 1 and 2. According to Gunter's Space Page and Wikipedia these two spacecrafts were built by Canopus Systems US (an affiliated of the Russian Dauria Aerospace), and follow the 6U CubeSat standard \cite{PerseusM_GunterSpace,PerseusM_Wiki}. Thus both have a mass of around $6\,\unit{kg}$ and a Sun synchronous orbit with an altitude of $606\,\unit{km}$ \cite{UCSDatabase2015}. Finally, Another example is the DX 1 (Dauria Experimental 1), a $27\,\unit{kg}$ spacecraft, with a size of 40 x 40 x 30 cm, also built by Dauria Aerospace \cite{DX1_GunterSpace}. Besides testing technology it also carries an AIS receiver.

% ---------------------------------------------

\paragraph{Aeneas}: The Aeneas nano satellite is aimed at tracking cargo containers (equipped with a $1\,\unit{W}$ Wifi type transceiver) around the world \cite{Aherne2011}. Developed by students of the University of Southern California/Space Engineering Research Center in partnership with iControl Inc. (the primary payload provider), it was launched in 2012 \cite{UCSDatabase2015}. The orbit is an ellipse with a periapsis of about $480\,\unit{kg}$.

The spacecraft is a modified 3U Colony I Cubesat (based on Pumpkin XS-25a CubeSat bus), weighting about $3\,\unit{kg}$. Besides the body mounted solar panels it has four deployable panels of ClydeSpace (UK), which deploy to a 90\textdegree angle to have sufficient power to fulfil the mission goals \cite{Aeneas_EOPortal}. Because a pointing accuracy better than 2\textdegree is needed, it also has an additional two axis digital sun sensor (SS-411, from Sinclair Interplanetary), and three, single axis, MEMS (Micro-Electro-Mechanical Systems) gyroscopes from Analog Devices (ADIS16260) to propagate the sun vector during eclipses. Two monopole whip antennas support two radios, a Microhard MHX425 transceiver (for telemetry and command, with a capacity of $115\,\unit{kbps}$), and a AstroDev Neon beacon. Finally, the previous processor was changed by two Microchip PIC24-based.

Together with the primary payload (a $0.5\,\unit{m}$ deployable antenna to track the signals from the containers), an experimental radiation hardened flight processor is tested, has a secondary payload \cite{Aherne2011}. The antenna is formed by 30 ribs and a central mast, where the transceiver is located. When packed it fits inside the payload section (10 x 10 x 16 cm), using a system of springs to deploy.

% ---------------------------------------------
% ---------------------------------------------

\begin{table}[htbp]
  \centering
  \caption{Summary of Small Satellites}
	\label{tab:Sum_SmallSat}
    \begin{tabular}{ccccc}
    \noalign{\smallskip}\hline\noalign{\smallskip}
    Satellite & Mass [kg] & Power [W] & Mission/Payload & Launch \\
    \noalign{\smallskip}\hline\noalign{\smallskip}
    COPPER 				& 1,3   & 2,0   	& Imager 										& 2013   \\
		Aeneas 				& 3   	& 2,0   	& Track cargo containers 		& 2012   \\
		Perseus M1/2 	& 6    	& 6  			& AIS System 								& 2014   \\
		NTS/CanX-6 		& 6.5   & 5.6  		& AIS System 								& 2008   \\
		AISSat-1 			& 6.5   & 0.967  	& AIS System 								& 2010   \\
    WNISAT-1 			& 10    & 12,6  	& Imager 										& 2013   \\
		AprizeSat 3/4	& 13   	& --  		& AIS System 								& 2009   \\
		AISat					& 14   	& 15  		& AIS System 								& 2014   \\
		VesselSat 1		& 29   	& --  		& AIS System 								& 2011   \\
    VesselSat 2		& 29   	& --  		& AIS System 								& 2012   \\
		M3MSat 				& 80    & 80,0  	& AIS System 								& 2015   \\
		exactView 1		& 98    & --  		& AIS System 								& 2012   \\
    \noalign{\smallskip}\hline\noalign{\smallskip}
    \end{tabular}
\end{table}

